Close to Home: Analyzing Urban Consumer Behavior and Consumption Space in Seoul

This study explores how the relatedness density of amenities influences consumer buying patterns, focusing on multi-purpose shopping preferences. Using Seoul's credit card data from 2018 to 2023, we find a clear preference for shopping at amenities close to consumers' residences, particularly for trips within a 2 km radius, where relatedness density significantly influences purchasing decisions. The COVID-19 pandemic initially reduced this effect at shorter distances but rebounded in 2023, suggesting a resilient return to pre-pandemic patterns, which vary over regions. Our findings highlight the resilience of local shopping preferences despite economic disruptions, underscoring the importance of amenity-relatedness in urban consumer behavior.

==> output/omega_base_year.tex <==

\begin{table}
\centering
\caption{}
\label{table:year}
\begin{tabular}{lcccccc}
   \tabularnewline \midrule \midrule
   Dependent Variable: & \multicolumn{6}{c}{$log(salescount)_{ijpt}$}\\
                        & All             & 2019            & 2020            & 2021            & 2022            & 2023 \\   
   Model:               & (1)             & (2)             & (3)             & (4)             & (5)             & (6)\\  
   \midrule
   \emph{Variables}\\
   $\omega_{ipt}$        & 0.0034          & 0.0029          & -0.0012         & 0.0063          & 0.0063          & 0.0018\\   
                        & (0.0033)        & (0.0047)        & (0.0036)        & (0.0047)        & (0.0047)        & (0.0031)\\   
   $log(distance)_{ij}$     & -0.1536$^{***}$ & -0.1638$^{***}$ & -0.1550$^{***}$ & -0.1500$^{***}$ & -0.1469$^{***}$ & -0.1524$^{***}$\\   
                        & (0.0006)        & (0.0021)        & (0.0008)        & (0.0008)        & (0.0007)        & (0.0005)\\   
   $\omega_{ipt} Xlog(distance)_{ij}$   & -0.1375$^{***}$ & -0.1427$^{***}$ & -0.1405$^{***}$ & -0.1359$^{***}$ & -0.1364$^{***}$ & -0.1335$^{***}$\\   
                        & (0.0021)        & (0.0038)        & (0.0030)        & (0.0021)        & (0.0022)        & (0.0024)\\   
   \midrule
   \emph{Fixed-effects}\\
   ID                   & Yes             & Yes             & Yes             & Yes             & Yes             & Yes\\  
   ID\_o                & Yes             & Yes             & Yes             & Yes             & Yes             & Yes\\  
   sectorCode           & Yes             & Yes             & Yes             & Yes             & Yes             & Yes\\  
   year                 & Yes             &                 &                 &                 &                 & \\  
   \midrule
   \emph{Fit statistics}\\
   Observations         & 166,461,440     & 33,292,288      & 33,292,288      & 33,292,288      & 33,292,288      & 33,292,288\\  
   R$^2$                & 0.04523         & 0.04455         & 0.04568         & 0.04534         & 0.04589         & 0.04585\\  
   Within R$^2$         & 0.04038         & 0.03877         & 0.04075         & 0.04071         & 0.04134         & 0.04114\\  
   \midrule \midrule
   \multicolumn{7}{l}{\emph{Clustered (ID \& ID\_o) standard-errors in parentheses}}\\
   \multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\
\end{tabular}
\end{table}

==> output/omega_type_distance.tex <==

\begin{table}[ht]
\centering
\caption{}
\captionsetup[table]{font = {stretch = 1.5}, labelfont=it}
\label{table:type_distance}
\begin{tabular}{lccccc}
   \tabularnewline \midrule \midrule
   Dependent Variable: & \multicolumn{5}{c}{$log(salescount)_{ijpt}$}\\
                        & type A          & typeB           & typeC           & typeD           & typeE \\   
   Model:               & (1)             & (2)             & (3)             & (4)             & (5)\\  
   \midrule
   \emph{Variables}\\
   $\omega_{ipt} $       & -0.0079$^{**}$  & -0.0088         & -0.0064$^{**}$  & 0.0162$^{***}$  & 0.0527$^{***}$\\   
                        & (0.0035)        & (0.0140)        & (0.0030)        & (0.0043)        & (0.0081)\\   
   $log(distance)_{ij}$     & -0.0654$^{***}$ & -0.1206$^{***}$ & -0.1664$^{***}$ & -0.1622$^{***}$ & -0.1583$^{***}$\\   
                        & (0.0099)        & (0.0064)        & (0.0033)        & (0.0027)        & (0.0105)\\   
   $\omega_{ipt}Xlog(distance)_{ij}$   & -0.0329$^{***}$ & -0.0923$^{***}$ & -0.1479$^{***}$ & -0.1568$^{***}$ & -0.1566$^{***}$\\   
                        & (0.0052)        & (0.0077)        & (0.0044)        & (0.0039)        & (0.0103)\\   
   \midrule
   \emph{Fixed-effects}\\
   Destination                   & Yes             & Yes             & Yes             & Yes             & Yes\\  
   Residence                & Yes             & Yes             & Yes             & Yes             & Yes\\  
   Amenity           & Yes             & Yes             & Yes             & Yes             & Yes\\  
   Year                 & Yes             & Yes             & Yes             & Yes             & Yes\\  
   \midrule
   \emph{Fit statistics}\\
   Observations         & 5,527,040       & 31,211,520      & 61,772,800      & 56,570,880      & 11,379,200\\  
   R$^2$                & 0.01615         & 0.02776         & 0.04998         & 0.05885         & 0.06467\\  
   Within R$^2$         & 0.00705         & 0.01581         & 0.04480         & 0.05470         & 0.05966\\  
   \midrule \midrule
   \multicolumn{6}{l}{\emph{Clustered (Destination \& Residence) standard-errors in parentheses}}\\
   \multicolumn{6}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\
\end{tabular}
\end{table}


==> output/omega_walkingtrip.tex <==

\begin{table}[ht]
\centering
\caption{}
\label{table:walkingtrip}
\begin{tabular}{lcccc}
   \tabularnewline \midrule \midrule
   Dependent Variable: & \multicolumn{4}{c}{$log(salescount)_{ijpt}$}\\
                         & All             & pre-Covid(2019) & Covid(2020-2022) & Recovery(2023) \\   
   Model:                & (1)             & (2)             & (3)              & (4)\\  
   \midrule
   \emph{Variables}\\
   $\omega_{ipt}$         & -0.0109$^{***}$ & -0.0081$^{**}$  & -0.0111$^{***}$  & -0.0133$^{***}$\\   
                         & (0.0023)        & (0.0039)        & (0.0026)         & (0.0019)\\   
   $walkingtripX\omega_{ipt}$  & 1.843$^{***}$   & 1.845$^{***}$   & 1.847$^{***}$    & 1.830$^{***}$\\   
                         & (0.0840)        & (0.0929)        & (0.0841)         & (0.0851)\\   
   \midrule
   \emph{Fixed-effects}\\
   Destination                    & Yes             & Yes             & Yes              & Yes\\  
   Residence                 & Yes             & Yes             & Yes              & Yes\\  
   Amenity            & Yes             & Yes             & Yes              & Yes\\  
   Year                  & Yes             & Yes             & Yes              & Yes\\  
   \midrule
   \emph{Fit statistics}\\
   Observations          & 166,461,440     & 33,292,288      & 99,876,864       & 33,292,288\\  
   R$^2$                 & 0.03134         & 0.02936         & 0.03200          & 0.03232\\  
   Within R$^2$          & 0.02643         & 0.02349         & 0.02724          & 0.02753\\  
   \midrule \midrule
   \multicolumn{5}{l}{\emph{Clustered (Destination \& Residence) standard-errors in parentheses}}\\
   \multicolumn{5}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\
\end{tabular}
\end{table}
